LLM-based Cognitive Models of Students with Misconceptions

Accurately modeling student cognition is crucial for developing effective AI-driven educational technologies. A key challenge is creating realistic student models that satisfy two essential properties: (1) accurately replicating specific misconceptions, and (2) correctly solving problems where these misconceptions are not applicable. This dual requirement reflects the complex nature of student understanding, where misconceptions coexist with correct knowledge. This paper investigates whether Large Language Models (LLMs) can be instruction-tuned to meet this dual requirement and effectively simulate student thinking in algebra. We introduce MalAlgoPy, a novel Python library that generates datasets reflecting authentic student solution patterns through a graph-based representation of algebraic problem-solving. Utilizing MalAlgoPy, we define and examine Cognitive Student Models (CSMs) - LLMs instruction tuned to faithfully emulate realistic student behavior. Our findings reveal that LLMs trained on misconception examples can efficiently learn to replicate errors. However, the training diminishes the model's ability to solve problems correctly, particularly for problem types where the misconceptions are not applicable, thus failing to satisfy second property of CSMs. We demonstrate that by carefully calibrating the ratio of correct to misconception examples in the training data - sometimes as low as 0.25 - it is possible to develop CSMs that satisfy both properties. Our insights enhance our understanding of AI-based student models and pave the way for effective adaptive learning systems.

==> figures/algos_old.tex <==
\begin{figure*}[th!]
\centering
\begin{minipage}[t]{0.32\textwidth}
\begin{algorithm}[H]
\small
\caption{Reduction Process}
\label{fig:algo1}
\begin{algorithmic}[1]
\Function{Reduce}{$e, T_i$}
    \If{$T_i = T_1$}
        \Return $e$
    \EndIf
    \State $e' \gets R_i(e)$
    \State $T_j \gets$ type of $e'$
    \If{$(T_i, T_k) \in E_M$ for some $T_k$}
        \State Choose between $(T_i, T_j)$ and $(T_i, T_k)$
        \State Update $e'$ and $T_j$ if misconception is chosen
    \EndIf
    \State \Return \Call{Reduce}{$e', T_j$}
\EndFunction
\end{algorithmic}
\end{algorithm}
\end{minipage}
\hfill
\begin{minipage}[t]{0.59\textwidth}
\begin{algorithm}[H]
\small
\caption{Reduction with Misconceptions}
\label{fig:algo2}
\begin{algorithmic}[1]
\Function{ReduceWithMisconceptions}{$e, T_i, \mathcal{M}$}
    \If{$T_i = T_1$}
        \Return $e$
    \EndIf
    \State $e' \gets R_i(e)$
    \State $T_j \gets$ type of $e'$
    \For{$M \in \mathcal{M}$}
        \If{$M(T_i, T_j) \in E_M$}
            \State $(T_i, T_k) \gets M(T_i, T_j)$
            \State $e'' \gets$ apply $M$ to $e'$
            \State \Return \Call{ReduceWithMisconceptions}{$e'', T_k, \mathcal{M}$}
        \EndIf
    \EndFor
    \State \Return \Call{ReduceWithMisconceptions}{$e', T_j, \mathcal{M}$}
\EndFunction
\end{algorithmic}
\end{algorithm}
\end{minipage}
\caption{Algorithms for algebraic equation reduction in MalAlgoPy: (left) Basic reduction process that transforms equations to simpler forms; (right) Extended reduction process that systematically applies a set of predefined misconceptions, generating both correct and incorrect solution paths. $\mathcal{M}$ is the set of all applicable misconceptions.}
\label{fig:algorithms}
\vspace{-3mm}
\end{figure*}

==> figures/legacy/misc_w_correct.tex <==
\begin{figure*}[t!]
\centering
\includegraphics[width=\linewidth]{figures/images/misconception_vs_correct_accuracy_strong_2plots.pdf} 
\hfill
\caption{Recovery of correct problem-solving abilities with introduction of correct examples. This graph shows how adding correct training examples alongside misconception examples helps the model regain correct solving accuracy. The rapid improvement suggests an effective method for creating balanced student models that can replicate misconceptions while retaining correct problem-solving skills.}
\label{fig:correct_solving_accuracy_two_plots}
\vspace{-5mm}
\end{figure*}

==> figures/legacy/split_acc.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{figures/images/avg_accuracy_A_vs_NA_2plots_no_base.pdf} 
\hfill
\caption{Impact of misconception learning on problem types applicable (A) and non-applicable (NA) to the misconception. Solid lines represent accuracy for types where the misconception is applicable, while dashed lines show types where it's not. The goal is to create a model that exhibits learned misconceptions for A problems while maintaining correct solving abilities for NA problems, mimicking real student behavior.}
\label{fig:avg_accuracy_A_vs_NA_4plots}
\end{figure*}

==> sections/contributions.tex <==
This paper presents two key contributions to the field of educational AI and cognitive modeling in mathematics:

We introduce MalAlgoPy, a novel Python library for generating cognitively faithful student solutions to algebraic problems. Building upon the seminal work of \citealp{malrules}, MalAlgoPy implements a formal graph-based representation of algebraic problem-solving. The library models 16 distinct problem types as nodes in a directed acyclic graph, with edges representing both correct transformations and misconceptions. This structure allows for the programmatic generation of solution paths through depth-first traversal, incorporating both correct steps and error patterns. MalAlgoPy formalizes misconceptions as functions that map correct edges to incorrect ones, enabling the systematic exploration of the solution space. This graph-theoretical approach provides a robust framework for studying student cognition and developing intelligent tutoring systems, capable of generating and analyzing a comprehensive set of possible solution strategies.

Using MalAlgoPy, we conduct a comprehensive study on training Large Language Models (LLMs) to simulate student cognitive processes in algebra. We introduce two types of cognitive agents:
a) Weak cognitive agents: Models that accurately replicate specific misconceptions but struggle with correct problem-solving.
b) Strong cognitive agents: Models that balance misconception replication with maintaining correct problem-solving abilities.
The latter are crucial for realistic student modeling, as they mirror actual student behavior where misconceptions coexist with correct understanding across different problem types. 
Our analysis presents scaling curves that reveal:
(i) The efficiency with which LLMs acquire mathematical misconceptions;
(ii) The trade-off between misconception accuracy and correct problem-solving ability in weak cognitive agents; and
(iii) The surprising ease of recovering correct problem-solving skills in strong cognitive agents with minimal additional training.
These findings lead to the establishment of scaling laws that quantify the relationship between training data, misconception accuracy, and correct problem-solving ability, providing insights into the development of more nuanced and educationally valuable AI systems.

==> tables/problem_types.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|l|l|}
\hline
\textbf{Type} & \textbf{Expression} & \textbf{Applicable Misconceptions} \\
\hline
T1 & $Ax = B$ & M19, M20\_S20, M21, M22\_S1 \\
T2 & $Ax = B + C$ & M14\_M15, M17\_M18, M19, M20\_S20, M21, M22\_S1 \\
T3 & $Ax = B * C$ & M16, M19, M20\_S20, M21, M22\_S1 \\
T4 & $Ax + Bx = C$ & M14\_M15, M17\_M18, M19, M20\_S20, M21, M22\_S1 \\
T5 & $Ax + B = C$ & M12\_S15\_M13, M19, M20\_S20, M21, M22\_S1 \\
T6 & $A + Bx = C$ & M12\_S15\_M13, M19, M20\_S20, M21, M22\_S1 \\
T7 & $Ax = Bx + C$ & M12\_S15\_M13, M19, M20\_S20, M21, M22\_S1 \\
T8 & $Ax = B(C*D)$ & M1, M4, M19, M20\_S20, M21, M22\_S1 \\
T9 & $Ax = B(Cx + D)$ & M1, M2\_S3, M5, M6, M8, M12\_S15\_M13, M19, M20\_S20, M21, M22\_S1 \\
T10 & $Ax = B + C * D$ & M1, M3, M16, M19, M20\_S20, M21, M22\_S1 \\
T11 & $A + Bx + Cx = D$ & M19, M20\_S20, M21, M22\_S1 \\
T12 & $Ax = B + C(Dx + E)$ & M1, M2\_S3, M3, M5, M6, M8, M12\_S15\_M13, M19, M20\_S20, M21, M22\_S1 \\
T14 & $Ax + B = Cx + D$ & M11, M19, M20\_S20, M21, M22\_S1 \\
\hline
\end{tabular}
}
\caption{Problem Types and Their Applicable Misconceptions}
\end{table*}
